PROBE: Benchmarking Code Generation in Large Language Models

Large Language Models (LLMs) are increasingly being used in everyday software engineering tasks, particularly in automated code generation. Despite their widespread adoption, these models remain far from perfect, making systematic and fair evaluation essential to understand their strengths and limitations. In the context of code generation, existing benchmarks are limited: they often target a single programming language and rely primarily on unit test outcomes, while overlooking other critical dimensions such as the overall quality of the generated code and its closeness to a valid solution. To address these gaps, we introduce PROBE, an extensible benchmark framework that, unlike prior work, establishes a systematic structure built on diverse and well-defined metrics, representative workloads, varied prompt templates, and a robust experimental procedure. In practice, the code generated by the LLMs is evaluated along three complementary dimensions: functional correctness, proximity to valid solutions, and code quality, enabling a comprehensive assessment of performance. We use PROBE to evaluate four open-source and two proprietary models under three prompting strategies across five programming languages. We further complement this analysis with a study of common errors in the code and provide concrete examples, offering clearer insight into where LLMs tend to struggle. Our findings show that, while LLMs achieve promising results, they struggle with harder problems and, in the case of smaller models, with programming languages that have fewer available resources for training, and they often fail due to fundamental and easily avoidable errors that underscore the unreliability of automatically generated code.

==> glossary.tex <==
\thispagestyle{plain}

\newacronym{os}{OS}{Operating System}
\newacronym{nyi}{NYI}{Not Yet Implemented}
\newacronym{dei}{DEI}{Department of Informatics Engineering}
%\newacronym{LLMs}{LLMs}{Large Language Model}
\newacronym{AI}{AI}{Artificial Intelligence}
\newacronym{BLEU}{BLEU}{Bilingual Evaluation Understudy}
\newacronym{ROUGE}{ROUGE}{Recall-Oriented Understudy for Gisting Evaluation}
\newacronym{METEOR}{METEOR}{Metric for Evaluation of Translation with Explicit ORdering}
\newacronym{ML}{ML}{Machine Learning}
\newacronym{NLP}{NLP}{Natural Language Processing}
\newacronym{ICL}{ICL}{In-Context Learning}
\newacronym{RAG}{RAG}{Retrieval Augmented Generation}
\newacronym{LSTM}{LSTM}{Long Short-Term Memory}
\newacronym{RNNs}{RNNs}{Recurrent Neural Networks}
\newacronym{BERT}{BERT}{Bidirectional Encoder Representations from Transformers}
\newacronym{MLM}{MLM}{Masked Language Modeling}
\newacronym{NSP}{NSP}{Next Sentence Prediction}
\newacronym{ASTs}{ASTs}{Abstract Syntax Trees}
\newacronym{MBPP}{MBPP}{Mostly Basic Python Problems}
\newacronym{RLHF}{RLHF}{Reinforcement Learning from Human Feedback}
\newacronym{GenAI}{GenAI}{Generative Artificial Intelligence}
\newacronym{CoT}{CoT}{Chain-of-Thought}
\newacronym{LLOC}{LLOC}{Logical Lines of Code}
\newacronym{SLOC}{SLOC}{Source Lines of Code}
\newacronym{LOC}{LOC}{Lines of Code}
\newacronym{MoE}{MoE}{Mixture of Experts}
\newacronym{GMM}{GMM}{Gaussian Mixture Models}
\newacronym{NLOC}{NLOC}{Number of Lines of Code}

\newglossaryentry{LLM}
{
  name={LLM},
  description={Large Language Model},
  first={Large Language Model (LLM)},
  plural={LLMs},
  descriptionplural={Large Language Models},
  firstplural={Large Language Models (LLMs)}
}

\thispagestyle{plain}
